Convergence and Recovery Guarantees of Unsupervised Neural Networks for Inverse Problems

Neural networks have become a prominent approach to solve inverse problems in recent years. While a plethora of such methods was developed to solve inverse problems empirically, we are still lacking clear theoretical guarantees for these methods. On the other hand, many works proved convergence to optimal solutions of neural networks in a more general setting using overparametrization as a way to control the Neural Tangent Kernel. In this work we investigate how to bridge these two worlds and we provide deterministic convergence and recovery guarantees for the class of unsupervised feedforward multilayer neural networks trained to solve inverse problems. We also derive overparametrization bounds under which a two-layers Deep Inverse Prior network with smooth activation function will benefit from our guarantees.

==> tex/sec_discrete_MSE.tex <==
\section{Discrete Case With MSE Loss}

Until now we provided results in the continuous gradient flow case, however in practice one has to use the discrete version of the algorithm, that is gradient descent. In this discrete version we consider update of the form
\begin{align}\label{eq:grad_descent}
    \thetav(\tau+1) = \thetav(\tau) - \gamma \nabla_{\thetavtau}\lossy(\yvtau)
\end{align}
where $\gamma$ is the chosen time step. If one chooses gamma infinitely small, it would become equivalent to the gradient flow equation~\eqref{eq:gradflow}. The question is then how should one choose $\gamma$ to ensure that all the results we found in Theorem~\ref{thm:main} remain valid. 

As a first approach to this discrete problem, we choose a simpler setting than the one of Theorem~\ref{thm:main}. We restrict ourselves to linear problems with forward operator $\fop\in\R^{m\times n}$ and we optimize the network using the MSE loss that is $\loss(\yv(\cdot)) = \norm{\yv(\cdot) - \yv}^2$. This implies that from the assumptions of Theorem~\ref{thm:main} we only need~\ref{ass:phi_diff} and that $\yv \in \ran{\fop}$ to reach the same set of assumptions. Indeed all the assumptions on the loss are met by the MSE and a linear operator obviously respects~\ref{ass:F_diff}.

We now have everything in place to present the results one can reach in the discrete setting:

% Define the theorem
\begin{theorem}\label{thm:main_discr}
    Consider a network $\gv(\uv,\cdot)$ with activation function such that \ref{ass:phi_diff} holds, a linear forward operator $\fop$ and the MSE loss $\lossy(\yv(\cdot)) = \norm{\yv(\cdot) - \yv}^2$. Let $\thetav(\cdot)$ be the parameters found at each iteration of \eqref{eq:grad_descent} where the initialization $\thetavz$ is such that
    \begin{equation}\label{eq:bndR2}
        \sigminjgz > 0 \qandq R' < R
    \end{equation}
    where R' and R obey
    \begin{equation}\label{eq:RandR'2}
        R' = \frac{4}{\sigminF\sigminjgz}\sqrt{\lossyzy} \qandq R = \frac{\sigminjgz}{2\Lip_{\Ball(\thetavz,R)}(\Jg)}. 
    \end{equation}
If $\gamma \leq \frac{1}{L}$ with $L = 2 \Lip_{\Ball(\thetavz,R)}(\Jg) \Lip_{\Ball(\thetavz,R)}(\gv) \norm{\fop}^2$, then the following holds:
\begin{enumerate}[label=(\roman*)]
\item \label{thm:main_y_bounded2} the loss converges to $0$ at the rate
\begin{align}\label{eq:lossrate2}
    \lossytauy &\leq \left( 1-\frac{\eta\sigminjgz^2\sigminA^2}{L}  \right)^\tau \lossy(\yvz)
\end{align}
with $\eta = \gamma L - \gamma^2L^2/2 \in [0,1/2]$. Moreover, $\thetav(\tau)$ converges to a global minimizer $\thetav_{\infty}$ of $\lossy(\fop\gv(\uv,\cdot))$, at the rate
\begin{align}\label{eq:thetarate2}
\norm{\thetav(\tau) - \thetav_{\infty}} &\leq \frac{4}{\sigminjgz\sigminA}\norm{\yvtau - \yv}.
\end{align}

\item Furthermore,
\begin{align}\label{eq:yrate_discr}
    \norm{\yvtau - \yvc} \leq 2\norm{\veps}  \quad \text{when} \quad \tau \geq \frac{2 \log(\norm{\veps}) - \log(\lossy(\yvz))}{\log\left(1 - \frac{\eta\sigminjgz^2\sigminA^2}{L}\right)}
\end{align}

\item Assume that 
\begin{assumption}\label{ass:A_inj}
$\muA > 0$ where
$
\displaystyle{\muA \eqdef \inf_{\xv \in \modifs{\Sigma'}} \frac{\norm{\fop(\xv-\xvcsigma)}}{\norm{\xv-\xvcsigma}} \modifs{\text{ with } \Sigma' \eqdef \Sigma_{\Ball(\thetavz,R')}}}.
$%\modifs{ with $\displaystyle{\Sigma' \eqdef \Sigma_{\Ball_{R'}(\thetavz)}$}
\end{assumption}
Then
\begin{align}\label{eq:xrate_discr}
\begin{split}
\norm{\xv(\tau) - \xvc} \leq \muA\inv \left( 1-\frac{\eta\sigminjgz^2\sigminA^2}{L}  \right)^{\tau/2}\sqrt{\lossyzy}  \\
+ \pa{1+\frac{\norm{\fop}}{\muA}}\dist(\xvc,\Sigma') + \frac{\norm{\veps}}{\muA}.
\end{split}
\end{align}

\end{enumerate}
\end{theorem}

% discussion Th

We derive from this theorem of the discrete case the same type of results as the ones in Theorem~\ref{thm:main}. It appears that to maintain the guarantees obtained in the continuous case, one need to ensures that $\gamma \leq \frac{1}{L}$ for an $L$-smooth function on $\Ball(\thetavz,R)$. This is in line with classical descent lemmas which use this smoothness property to ensure that~\eqref{eq:grad_descent} is a descent and will reach a minimizer of the function. We combine this with the constraint on the initialization to ensure that it is a global minimizer.

This allows us to keep the condition on the initialisation the same as the one in Theorem~\ref{thm:main}. From~\eqref{eq:lossrate2} we have that the loss converges at a geometric rate which correspond to the continuous case of~\eqref{eq:lossrate}. The difference lies in the impact of $\gamma$ on this rate. The optimal rate is obtained when $\gamma = \frac{1}{L}$ which indicates that $\eta$ is maximised at $1/2$. However as long as one ensures that $\gamma$ is smaller than this optimal point, the loss will converge to an optimal solution although at a slower rate.

The other results~\eqref{eq:yrate_discr} and~\eqref{eq:xrate_discr} are almost exactly the same as their counterpart in Theorem~\ref{thm:main} which is to be expected as both results relies on~\eqref{eq:lossrate} to hold. Once we prove~\eqref{eq:lossrate2}, it is straightforward to obtain the other two results by following the same line of proof adapted to our discrete setting.

% Proof
\section{Proofs}
We first present useful lemmas that will help us prove the claims from Theorem~\ref{thm:main_discr}.

\begin{lemma}\label{lemma:descent_trajectory}
    If $\thetav(\cdot) \in \Ball(\thetavz,R)$, choosing a step size of $\gamma \leq 1/L$ with $L = 2 \Lip_{\Ball(\thetavz,R)}(\Jg) \Lip_{\Ball(\thetavz,R)}(\gv) \norm{\fop}^2$ ensures that $\lossy(\cdot)$ is non-increasing and thus converges
\end{lemma}
\begin{proof}
    % We first recall a very classical result about gradient descent of L-smooth functions. Let's assume that $f$ is an L-smooth function, then by the fundamental theorem of calculus we have
    % \begin{align*}
    %     f(a) - f(b) &= \int_{a}^{b}\deriv{f(s)}{s}ds\\
    %     &= \int_0^1\deriv{f(b + t(a - b))}{(b + t(a - b))}(a - b)dt.
    % \end{align*}

    % By subtracting a constant and taking the absolute value we obtain
    % \begin{align*}
    %     \abs{f(a) - f(b) - \nabla_{b}\tp f(b)(a - b)} &= \abs{\int_0^1 (\nabla_{b + t(a - b)}f(b + t(a - b)) - \nabla_{b}f(b))\tp(a - b)dt}\\
    %     &\leq \int_0^1 Lt\norm{a - b}^2 dt = \frac{L}{2}\norm{a - b}^2
    % \end{align*}
    % where we use the L-smoothness of the loss function. Let's now say that  $a = \yvtauplus$ and $b = \yvtau$ and recall that by definition $a - b = - \gamma \nabla_{\thetavtau}\lossy(\yvtau)$. This leads to
    We first recall a very classical result about gradient descent of L-smooth functions. Let us assume that $\lossy$ is L-smooth and define $b_\delta = a + \delta(b-a)$, then by the fundamental theorem of calculus we have
    \begin{align*}
        \lossy(\yv(a)) - \lossy(\yv(b)) &= \int_{\thetav(a)}^{\thetav(b)}\nabla_{\thetavs}\lossy(\yv(s))\tp ds\\
        &= \int_0^1\nabla_{\thetav(b_\delta)}\lossy(\yv(b_\delta))\tp(\thetav(a) - \thetav(b))d\delta.
    \end{align*}

    By subtracting a constant and taking the absolute value we obtain
    \begin{align*}
        \abs{\lossy(\yv(a)) - \lossy(\yv(b)) - \nabla_{\thetav(b)}\lossy(b)\tp(\thetav(a) - \thetav(b))} &= \abs{\int_0^1 (\nabla_{\thetav(b_\delta)}\lossy(\yv(b_\delta)) - \nabla_{\thetav(b)}\lossy(\yv(b)))\tp(\thetav(a) - \thetav(b))d\delta}\\
        &\leq \int_0^1 L\delta\norm{\thetav(a) - \thetav(b)}^2 d\delta = \frac{L}{2}\norm{\thetav(a) - \thetav(b)}^2
    \end{align*}
    where we use the L-smoothness of the loss function. Let's now say that $a = \tau + 1$ and $b = \tau$ and recall that by definition $\thetav(a) - \thetav(b) = - \gamma \nabla_{\thetavtau}\lossy(\yvtau)$. This leads to
    \begin{align}\label{eq:diff_step_descent}
        \lossy(\yvtauplus) - \lossy(\yvtau) + \gamma\norm{\nabla_{\thetavtau}\lossy(\yvtau)}^2 \leq \frac{L\gamma^2}{2}\norm{\nabla_{\thetavtau}\lossy(\yvtau)}^2 \nonumber \\
         \lossy(\yvtauplus) - \lossy(\yvtau) \leq (\frac{L\gamma^2}{2} - \gamma) \norm{\nabla_{\thetavtau}\lossy(\yvtau)}^2.
    \end{align}
    Now, let us say that $\gamma = \frac{\lambda}{L}$ with $\lambda \in ]0,1]$, we get
    \begin{align}\label{eq:descent_nonincr}
        \lossy(\yvtauplus) - \lossy(\yvtau) \leq -\frac{1}{\beta L} \norm{\nabla_{\thetavtau}\lossy(\yvtau)}^2,
    \end{align}
    where $\beta = \frac{1}{(1 - \lambda/2)\lambda} \in [2,+\infty[$, which ensures that the process is indeed a descent and that $\lossy(\cdot)$ is non-increasing w.r.t $\tau$.

    We now have to show that $\lossy$ is indeed a smooth function. Since in our setting $\lossy$ is the MSE we have
    \begin{align}\label{eq:gradthetaloss}
        \nabla_{\thetavtau}\lossy(\yvtau) = 2\Jg(\thetavtau)\tp\fop\tp(\yv(\tau) - \yv).
    \end{align}
    We know that $\gv$ is Lipschitz continuous as it is a composition of Lipschitz operators (linear layers or Lipschitz activation functions by \ref{ass:phi_diff}), which means that $\Jg$ is also Lipschitz continuous. Using the assumption that $\thetav(\cdot) \in \Ball(\thetavz,R)$ we obtain
    \begin{align*}
        \norm{\nabla_{\thetav(a)}\lossy(\yv(a)) - \nabla_{\thetav(b)}\lossy(\yv(b))} &\leq 2 \Lip_{\Ball(\thetavz,R)}(\Jg) \norm{\fop} \norm{\yv(a) - \yv(b)}\\
        &\leq 2 \Lip_{\Ball(\thetavz,R)}(\Jg) \Lip_{\Ball(\thetavz,R)}(\gv) \norm{\fop}^2 \norm{\thetav(a) - \thetav(b)},
    \end{align*}
    which conclude that $\lossy$ is $L$-smooth with $L = 2 \Lip_{\Ball(\thetavz,R)}(\Jg) \Lip_{\Ball(\thetavz,R)}(\gv) \norm{\fop}^2$.
\end{proof}

\begin{lemma}\label{lemma:link_params_singvals_discr}
Assume \ref{ass:phi_diff} holds. Recall $R$ and $R'$ from \eqref{eq:RandR'2}. Let $\thetav(\cdot)$ be a solution of \eqref{eq:grad_descent}.
    \begin{enumerate}[label=(\roman*)]
        \item \label{claim:singvals_bounded_if_params_bounded_discr} If $\thetav \in \Ball(\thetavz,R)$ then
        \begin{align*}
            \sigmin(\jtheta) \geq \sigminjgz/2.
        \end{align*}
        
        \item  \label{claim:params_bounded_if_singvals_bounded_discr} If the loss is $L$-smooth on $\Ball(\thetavz,R')$ and $\gamma \leq \frac{1}{L}$, then if for all $s \in {0,...,\tau}$, $\sigminjgs \geq \frac{\sigminjgz}{2}$ we have
            \begin{align*}
                \thetavt \in \Ball(\thetavz,R').
            \end{align*}
        
        \item \label{claim:sigval_bounded_everywhere_discr}
        If $R'<R$, then for all $t \geq 0$, $\sigminjgt \geq \sigminjgz/2$.
\end{enumerate}
\end{lemma}
\begin{proof}
We reuse the same proof as in Lemma~\ref{lemma:link_params_singvals} except for~\ref{claim:params_bounded_if_singvals_bounded_discr} that we now prove.
We know that $\gv$ is Lipschitz and that the loss is also locally Lipschitz which permit us to assume that there exists an $L'$ such that the loss is $L'$-smooth on the trajectory of $\thetav(\cdot)$ with $L'$ potentially very large. We thus take for now $\gamma = \lambda/L'$ with $\lambda\in]0,1]$. This allows us to use \eqref{eq:descent_nonincr} and the fact that $\left(a - \frac{b}{2a}\right)^2 \geq a^2 - b$ to obtain that
    \begin{align}
        \norm{\yv(\tau+1) - \yv}^2 &\leq \norm{\yv(\tau) - \yv}^2 - \frac{\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}^2}{\beta L'} \nonumber\\ \label{eq:square_comp}
        &\leq \left(\norm{\yv(\tau) - \yv} - \frac{\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}^2}{2\beta L'\norm{\yv(\tau) - \yv}} \right)^2.
    \end{align}
    We now define the Lyapunov function 
    \begin{align}\label{eq:lyapu_discr}
        V(\tau) = \norm{\yv(\tau) - \yv} + \alpha\sum_{i=0}^{k-1}\norm{\thetav(i+1) - \thetav(i)},
    \end{align}
    and show that it is non-increasing when $\alpha = \frac{\sigminjgz\sigminA}{4}$. We recall 
    \begin{align*}
        V(\tau + 1) - V(\tau) &= \norm{\yv(\tau+1) - \yv} - \norm{\yv(\tau) - \yv} + \alpha\norm{\thetav(\tau+1) - \thetav(\tau)}\\
        {\small \eqref{eq:square_comp}} &\leq - \frac{\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}^2}{2\beta L'\norm{\yv(\tau) - \yv}} + \gamma\alpha\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}\\
        &= \frac{\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}}{L'}\left( \alpha\lambda - \frac{\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}}{2\beta\norm{\yv(\tau) - \yv}}\right)\\
        {\small (a)}&\leq \frac{\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}}{L'} \left( \alpha\lambda - \frac{\sigminjgz\sigminA}{2\beta} \right)\\
        &\leq \frac{\norm{\nabla_{\thetav(\tau)}\lossy(\yvtau)}}{\lambda L'} \left( \alpha - \frac{(2 - \lambda)\sigminjgz\sigminA}{4} \right)\\
        &\leq 0
    \end{align*}
    where we used in $(a)$ that $\sigmin(\Jg(\tau)) > \frac{\sigminjgz}{2}$. This result means that with the chosen $\alpha$, we have that for any $\tau \geq 0$, $V(\tau)\leq V(0)$, which in turn allows us to obtain that 
    \begin{align*}
        \norm{\thetav(\tau) - \thetavz} \leq \sum_{i=0}^{\tau - 1}\norm{\thetav(i+1) - \thetav(i)} \leq \frac{1}{\alpha}\norm{\yv(0) - \yv}
    \end{align*}
    which informs us that $\thetav(\cdot) \in \Ball(\thetavz,R')$. Since this bound exists, we only require smoothness of the loss on $\Ball(\thetavz,R')$. Let's say that the loss is $L$-smooth on this ball, then we do not need $\gamma = \lambda/L'$ but only $\gamma = \lambda/L$ for our results to hold which concludes the proof.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:main_discr}]
\begin{enumerate}[label=(\roman*)]
\item Due to~\eqref{eq:bndR2}, Lemma~\ref{lemma:link_params_singvals_discr}~\ref{claim:sigval_bounded_everywhere_discr} and~\ref{claim:params_bounded_if_singvals_bounded_discr} ensuring that $\thetav(\cdot) \in \Ball(\thetavz,R')$. Now using Lemma~\ref{lemma:descent_trajectory} and that $\gamma\leq\frac{1}{L}$, we have that the trajectory of~\eqref{eq:grad_descent} is a descent. Embarking from~\ref{eq:diff_step_descent} and recalling $\eta$ from the Theorem we obtain that
    \begin{align*}
        \lossy(\yvtauplus) - \lossy(\yvtau) &\leq (\frac{L\gamma^2}{2} - \gamma) \norm{\nabla_{\thetavtau}\lossy(\yvtau)}^2\\
        &\leq - \frac{\eta}{L}\norm{\nabla_{\thetavtau}\lossy(\yvtau)}^2.
    \end{align*}
    We use Lemma~\ref{lemma:link_params_singvals_discr}~\ref{claim:singvals_bounded_if_params_bounded_discr} that informs us that for all $\tau$, $\sigmin(\Jg(\tau)) \geq \frac{\sigminjgz}{2}$ and that $\yvtau - \yv \in \ran{\fop}$ to get
    \begin{align*}
        \lossy(\yvtauplus) - \lossy(\yvtau) &\leq - \frac{\eta\sigminjgz^2\sigminA^2}{L}\lossy(\yvtau)\\
        \lossy(\yvtauplus) &\leq \left(1 - \frac{\eta\sigminjgz^2\sigminA^2}{L} \right)\lossy(\yvtau)\\
        \lossy(\yvtauplus) &\leq \left(1 - \frac{\eta\sigminjgz^2\sigminA^2}{L} \right)^\tau\lossy(\yvz)\\
    \end{align*}
    which proves \eqref{eq:lossrate2}. 

    Since \eqref{eq:grad_descent} is a descent under the condition of the theorem, the parameters $\thetav(\cdot)$ will converge to some parameters $\thetav_\infty$ which is a global minimizer of the loss by~\eqref{eq:lossrate2}.  By using Lemma~\ref{lemma:link_params_singvals_discr}~\ref{claim:params_bounded_if_singvals_bounded_discr}, we know that the Lyapunov function~\eqref{eq:lyapu_discr} is non-increasing for $\alpha = \frac{\sigminjgz\sigminA}{4}$. Thus we have
    \begin{align*}
        V(\infty) - V(\tau) = \norm{\yv(\infty) - \yv} - \norm{\yv(\tau) - \yv} + \alpha\sum_{i=\tau}^{\infty} \norm{\thetav(i+1) - \thetav(i)} \leq 0.
    \end{align*}
    Using~\eqref{eq:lossrate2} which states that the loss converges to 0, we obtain
    \begin{align*}
        \norm{\thetav(\tau) - \thetav_\infty} \leq \sum_{i=\tau}^{\infty} \norm{\thetav(i+1) - \thetav(i)} \leq \frac{\norm{\yv(\tau) - \yv}}{\alpha}
    \end{align*}
    which proves~\eqref{eq:thetarate2}.

    \item By continuity of $\fop$ and $\gv(\uv,\cdot)$, we infer that $\yv(\cdot)$ also converges to $\yv_\infty$. By continuity of $\lossy(\cdot)$ and~\ref{eq:lossrate2} we have
    \begin{align*}
        0 = \lim_{\tau\to +\infty}\lossy(\yv(\tau)) = \lossy(\yv_\infty).
    \end{align*}
    From here we observe that
    \begin{align*}
        \norm{\yv(\tau) - \yvc} &\leq \norm{\yv(\tau) - \yv} + \norm{\veps}\\
        &\leq \sqrt{\lossy(\yv(\tau))} + \norm{\veps}\\
        &\leq \sqrt{\left(1-\frac{\eta\sigminjgz^2\sigminA^2}{L}\right)} + \norm{\veps}.
    \end{align*}
    It then appears that $\lossy(\yv(\tau)) \leq \norm{\veps}$ when $\tau \geq \frac{2 \log(\norm{\veps}) - \log(\lossy(\yvz))}{\log\left(1 - \frac{\eta\sigminjgz^2\sigminA^2}{L}\right)}$.

    \item We reuse the inequality from the proof of Theorem~\ref{thm:main} as the logic is the exact same. By Lemma~\ref{lemma:link_params_singvals_discr}, we have that $\thetav(\tau)\in\Ball(\thetavz,R')$, which entails that $\xv(\tau) \in \Sigma'$ for all $\tau\geq 0$. We obatin the following chain of inequalities:
    \begin{align*}
        \norm{\xv(\tau) - \xvc} &\leq  \norm{\xv(\tau) - \xvcsigma} + \dist(\xvc,\Sigma')\\
        {\small \ref{ass:A_inj}} &\leq \muA\inv \norm{\yv(\tau) - \fop\xvcsigma} + \dist(\xvc,\Sigma')\\
        &\leq \muA\inv \left( \norm{\yv(\tau) - \yv} + \norm{\yv - \fop\xvc} + \norm{\fop(\xvc - \xvcsigma)} \right) + \dist(\xvc,\Sigma')\\
        {\small \ref{eq:grad_descent},\ref{eq:lossrate2}}&\leq \muA\inv \left( 1-\frac{\eta\sigminjgz^2\sigminA^2}{L}  \right)^{\tau/2}\sqrt{\lossyzy}\\
        &\quad+\pa{1+\frac{\norm{\fop}}{\muA}}\dist(\xvc,\Sigma') + \frac{\norm{\veps}}{\muA},
    \end{align*}
    Finishing the proof of Theorem~\ref{thm:main_discr}.
\end{enumerate}
\end{proof}

